Using session types as an effect system

Side effects are a core part of practical programming. However, they are often hard to reason about, particularly in a concurrent setting. We propose a foundation for reasoning about concurrent side effects using sessions. Primarily, we show that session types are expressive enough to encode an effect system for stateful processes. This is formalised via an effect-preserving encoding of a simple imperative language with an effect system into the pi-calculus with session primitives and session types (into which we encode effect specifications). This result goes towards showing a connection between the expressivity of session types and effect systems. We briefly discuss how the encoding could be extended and applied to reason about and control concurrent side effects.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{S. J. Gay and J. Alglave (Eds.): Programming Language Approaches to\\ Concurrency- and Communication-Centric Software (PLACES 2015).\\
EPTCS 203, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.203.1}{10.4204/EPTCS.203.1}}
\pdfoutput=1

